RePD: Defending Jailbreak Attack through a Retrieval-based Prompt Decomposition Process

In this study, we introduce RePD, an innovative attack Retrieval-based Prompt Decomposition framework designed to mitigate the risk of jailbreak attacks on large language models (LLMs). Despite rigorous pretraining and finetuning focused on ethical alignment, LLMs are still susceptible to jailbreak exploits. RePD operates on a one-shot learning model, wherein it accesses a database of pre-collected jailbreak prompt templates to identify and decompose harmful inquiries embedded within user prompts. This process involves integrating the decomposition of the jailbreak prompt into the user's original query into a one-shot learning example to effectively teach the LLM to discern and separate malicious components. Consequently, the LLM is equipped to first neutralize any potentially harmful elements before addressing the user's prompt in a manner that aligns with its ethical guidelines. RePD is versatile and compatible with a variety of open-source LLMs acting as agents. Through comprehensive experimentation with both harmful and benign prompts, we have demonstrated the efficacy of our proposed RePD in enhancing the resilience of LLMs against jailbreak attacks, without compromising their performance in responding to typical user requests.

==> sections/99-archived.tex <==
\begin{wrapfigure}{r}{0.5\textwidth}
  \begin{subfigure}{.5\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/box-random-ASR-Vicuna-1.5-.pdf}
    \caption{A}
  \end{subfigure}%
  \begin{subfigure}{.5\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/box-random-ASR-Vicuna-1.5-.pdf}
    \caption{B}
  \end{subfigure}
  \caption{
  Evaluation of \sysname's performance on random generation and static generation.
  }
  \label{fig:random}
  \vspace{0.2in}
\end{wrapfigure}

\begin{figure}[!htp]%{r}{0.5\textwidth}
  \begin{subfigure}{\textwidth}
    \centering
    \includegraphics[width=0.25\textwidth]{figures/box-multi-ASR-Vicuna-1.5-.pdf}
    \caption{A}
  \end{subfigure}%
  \begin{subfigure}{0.25\textwidth}
    \centering
    \includegraphics[width=0.25\textwidth]{figures/box-multi-FPR-Vicuna-1.5-.pdf}
    \caption{B}
  \end{subfigure}
  \\
  \begin{subfigure}{0.25\textwidth}
    \centering
    \includegraphics[width=0.25\textwidth]{figures/box-multi-ASR-Llama-2-.pdf}
    \caption{A}
  \end{subfigure}%
  \begin{subfigure}{0.25\textwidth}
    \centering
    \includegraphics[width=0.25\textwidth]{figures/box-multi-FPR-Llama-2-.pdf}
    \caption{B}
  \end{subfigure}  
  \\
  \caption{
  Evaluation of \sysname's performance on single agent and multi-agents.
  }
  \label{fig:multi}
  \vspace{0.2in}
\end{figure}

\begin{table}[]
    \centering
    \begin{tabular}{l|l|rrrrrr}
    
    \toprule
    Model &         Framework &   AutoDAN &      PAIR &       GCG &       TAP &    Base64 &       LRL \\
    \hline\hline
    
    \multirow{4}{*}{Vicuna-7B} &     Self Reminder &     0.99 &  0.99 &  0.99 &  0.99 &    0.96 &  0.58 \\
     &       Safe Prompt &     0.99 &  0.87 &  0.99 &  0.50 &    0.49 &  0.22 \\
     &  GPT Paraphrasing &     0.71 &  0.52 &  0.40 &  0.27 &    0.28 &  0.27 \\
     &         \sysname &     0.44 &  0.19 &  0.25 &  0.27 &    0.26 &  0.14 \\
     &  \sysname-M &     0.06 &  0.05 &  0.08 &  0.00 &    0.08 &  0.11 \\
     \hline
    \multirow{4}{*}{Vicuna-13B} &     Self Reminder &     0.67 &  0.99 &  0.99 &  0.72 &    0.28 &  0.53 \\
     &       Safe Prompt &     0.99 &  0.75 &  0.83 &  0.30 &    0.70 &  0.21 \\
     &  GPT Paraphrasing &     0.46 &  0.30 &  0.37 &  0.33 &    0.19 &  0.24 \\
     &         \sysname &     0.28 &  0.28 &  0.14 &  0.14 &    0.16 &  0.11 \\
     &  \sysname-M &     0.03 &  0.04 &  0.09 &  0.07 &    0.06 &  0.07 \\
     \hline
    \multirow{4}{*}{Vicuna-33B} &     Self Reminder &     0.79 &  0.46 &  0.24 &  0.37 &    0.52 &  0.17 \\
     &       Safe Prompt &     0.38 &  0.38 &  0.36 &  0.51 &    0.13 &  0.12 \\
     &  GPT Paraphrasing &     0.26 &  0.46 &  0.17 &  0.23 &    0.18 &  0.09 \\
     &         \sysname &     0.12 &  0.18 &  0.17 &  0.09 &    0.10 &  0.09 \\
     &  \sysname-M &     0.03 &  0.00 &  0.02 &  0.05 &    0.05 &  0.06 \\
     \hline
    \multirow{4}{*}{Llama-7B} &     Self Reminder &     0.67 &  0.56 &  1.00 &  0.80 &    0.90 &  0.23 \\
     &       Safe Prompt &     1.00 &  0.58 &  0.48 &  0.81 &    0.18 &  0.38 \\
     &  GPT Paraphrasing &     0.40 &  0.22 &  0.25 &  0.18 &    0.28 &  0.10 \\
     &         \sysname &     0.13 &  0.18 &  0.13 &  0.12 &    0.14 &  0.09 \\
     &  \sysname-M &     0.00 &  0.00 &  0.01 &  0.00 &    0.02 &  0.04 \\
     \hline
     \multirow{4}{*}{Llama-13B} &     Self Reminder &     1.00 &  0.62 &  1.00 &  0.80 &    0.34 &  0.22 \\
     &       Safe Prompt &     1.00 &  0.52 &  0.30 &  0.56 &    0.27 &  0.06 \\
     &  GPT Paraphrasing &     0.24 &  0.25 &  0.28 &  0.29 &    0.07 &  0.07 \\
     &         \sysname &     0.12 &  0.21 &  0.09 &  0.14 &    0.05 &  0.04 \\
     &  \sysname-M &     0.00 &  0.03 &  0.01 &  0.00 &    0.03 &  0.03 \\
     \hline
    \multirow{4}{*}{Llama-70B} &     Self Reminder &     0.98 &  0.30 &  0.32 &  0.22 &    0.13 &  0.15 \\
     &       Safe Prompt &     0.24 &  0.58 &  0.20 &  0.16 &    0.11 &  0.07 \\
     &  GPT Paraphrasing &     0.14 &  0.08 &  0.08 &  0.12 &    0.05 &  0.03 \\
     &         \sysname &     0.07 &  0.04 &  0.04 &  0.04 &    0.04 &  0.02 \\
     &  \sysname-M &     0.01 &  0.01 &  0.02 &  0.00 &    0.02 &  0.02 \\
    \hline\hline
    
    \end{tabular}
    \caption{The detailed ASR of the evaluation.}
    \label{tab:asr_detail}
\end{table}


\begin{table}[]
    \centering
    \begin{tabular}{l|l|rrrrrr}
    \toprule
    Model &         Framework &  AutoDAN &  PAIR &   GCG &   TAP &  Base64 &   LRL \\
    \hline\hline
    
    \multirow{4}{*}{Vicuna-7B} &     Self Reminder &     0.04 &  0.04 &  0.04 &  0.04 &    0.04 &  0.04 \\
     &       Safe Prompt &     0.08 &  0.12 &  0.12 &  0.07 &    0.07 &  0.12 \\
     &  GPT Paraphrasing &     0.08 &  0.14 &  0.11 &  0.13 &    0.10 &  0.10 \\
     &         \sysname &     0.05 &  0.04 &  0.04 &  0.07 &    0.04 &  0.04 \\
     &  \sysname-M &     0.00 &  0.04 &  0.02 &  0.02 &    0.02 &  0.00 \\
     \hline
    \multirow{4}{*}{Vicuna-13B} &     Self Reminder &     0.04 &  0.04 &  0.04 &  0.04 &    0.04 &  0.04 \\
     &       Safe Prompt &     0.05 &  0.08 &  0.07 &  0.06 &    0.05 &  0.08 \\
     &  GPT Paraphrasing &     0.15 &  0.08 &  0.15 &  0.14 &    0.08 &  0.09 \\
     &         \sysname &     0.04 &  0.06 &  0.08 &  0.07 &    0.06 &  0.04 \\
     &  \sysname-M &     0.02 &  0.01 &  0.01 &  0.01 &    0.02 &  0.04 \\
      \hline
    \multirow{4}{*}{Vicuna-33B} &     Self Reminder &     0.01 &  0.01 &  0.01 &  0.01 &    0.01 &  0.01 \\
     &       Safe Prompt &     0.03 &  0.02 &  0.03 &  0.02 &    0.03 &  0.02 \\
     &  GPT Paraphrasing &     0.05 &  0.03 &  0.04 &  0.04 &    0.06 &  0.04 \\
     &         \sysname &     0.04 &  0.01 &  0.01 &  0.04 &    0.02 &  0.03 \\
     &  \sysname-M &     0.01 &  0.01 &  0.01 &  0.00 &    0.00 &  0.00 \\
     \hline
    \multirow{4}{*}{Llama-7B} &     Self Reminder &     0.01 &  0.01 &  0.01 &  0.01 &    0.01 &  0.01 \\
     &       Safe Prompt &     0.08 &  0.06 &  0.03 &  0.03 &    0.04 &  0.07 \\
     &  GPT Paraphrasing &     0.08 &  0.04 &  0.05 &  0.18 &    0.06 &  0.10 \\
     &         \sysname &     0.03 &  0.01 &  0.03 &  0.01 &    0.03 &  0.06 \\
     &  \sysname-M &     0.00 &  0.00 &  0.00 &  0.00 &    0.00 &  0.00 \\
     \hline
    \multirow{4}{*}{Llama-13B} &     Self Reminder &     0.01 &  0.01 &  0.01 &  0.01 &    0.01 &  0.01 \\
     &       Safe Prompt &     0.03 &  0.04 &  0.04 &  0.03 &    0.02 &  0.04 \\
     &  GPT Paraphrasing &     0.03 &  0.03 &  0.08 &  0.05 &    0.05 &  0.04 \\
     &         \sysname &     0.01 &  0.01 &  0.01 &  0.01 &    0.01 &  0.01 \\
     &  \sysname-M &     0.01 &  0.01 &  0.00 &  0.00 &    0.00 &  0.01 \\
     \hline
    \multirow{4}{*}{Llama-70B} &     Self Reminder &     0.01 &  0.01 &  0.01 &  0.01 &    0.01 &  0.01 \\
     &       Safe Prompt &     0.01 &  0.02 &  0.02 &  0.03 &    0.02 &  0.01 \\
     &  GPT Paraphrasing &     0.03 &  0.02 &  0.03 &  0.03 &    0.02 &  0.02 \\
     &         \sysname &     0.01 &  0.01 &  0.01 &  0.01 &    0.01 &  0.01 \\
     &  \sysname-M &     0.00 &  0.00 &  0.00 &  0.00 &    0.00 &  0.01 \\
    \hline\hline
    \end{tabular}
    \caption{The detailed FPR of the evaluation}
    \label{tab:fpr_details}
\end{table}

\begin{table}[]
    \centering
    \begin{tabular}{l|l|rrrrrr}
\toprule
Model &         Framework &  AutoDAN &  PAIR &   GCG &   TAP &  Base64 &   LRL \\
\hline\hline
\multirow{4}{*}{Vicuna-7B} &     Self Reminder &     0.48 &  0.48 &  0.48 &  0.48 &    0.50 &  0.69 \\
 &       Safe Prompt &     0.47 &  0.51 &  0.45 &  0.71 &    0.72 &  0.83 \\
 &  GPT Paraphrasing &     0.61 &  0.67 &  0.75 &  0.80 &    0.81 &  0.81 \\
 &         \sysname &     0.75 &  0.88 &  0.86 &  0.83 &    0.85 &  0.91 \\
 &  \sysname-M &     0.97 &  0.96 &  0.95 &  0.99 &    0.95 &  0.94 \\
 \hline
\multirow{4}{*}{Vicuna-13B} &     Self Reminder &     0.65 &  0.49 &  0.49 &  0.62 &    0.84 &  0.72 \\
 &       Safe Prompt &     0.48 &  0.59 &  0.55 &  0.82 &    0.62 &  0.86 \\
 &  GPT Paraphrasing &     0.69 &  0.81 &  0.74 &  0.77 &    0.86 &  0.84 \\
 &         \sysname &     0.84 &  0.83 &  0.89 &  0.90 &    0.89 &  0.92 \\
 &  \sysname-M &     0.97 &  0.97 &  0.95 &  0.96 &    0.96 &  0.95 \\
 \hline
\multirow{4}{*}{Vicuna-33B} &     Self Reminder &     0.60 &  0.76 &  0.87 &  0.81 &    0.73 &  0.91 \\
 &       Safe Prompt &     0.80 &  0.80 &  0.80 &  0.73 &    0.92 &  0.93 \\
 &  GPT Paraphrasing &     0.85 &  0.76 &  0.90 &  0.87 &    0.88 &  0.94 \\
 &         \sysname &     0.92 &  0.90 &  0.91 &  0.94 &    0.94 &  0.94 \\
 &  \sysname-M &     0.98 &  1.00 &  0.99 &  0.97 &    0.97 &  0.97 \\
 \hline
\multirow{4}{*}{Llama-7B} &     Self Reminder &     0.66 &  0.72 &  0.50 &  0.60 &    0.55 &  0.88 \\
 &       Safe Prompt &     0.46 &  0.68 &  0.75 &  0.58 &    0.89 &  0.78 \\
 &  GPT Paraphrasing &     0.76 &  0.87 &  0.85 &  0.82 &    0.83 &  0.90 \\
 &         \sysname &     0.92 &  0.91 &  0.92 &  0.94 &    0.92 &  0.92 \\
 &  \sysname-M &     1.00 &  1.00 &  1.00 &  1.00 &    0.99 &  0.98 \\
 \hline
\multirow{4}{*}{Llama-13B} &     Self Reminder &     0.49 &  0.69 &  0.49 &  0.60 &    0.82 &  0.89 \\
 &       Safe Prompt &     0.49 &  0.72 &  0.83 &  0.70 &    0.86 &  0.95 \\
 &  GPT Paraphrasing &     0.87 &  0.86 &  0.82 &  0.83 &    0.94 &  0.94 \\
 &         \sysname &     0.93 &  0.89 &  0.95 &  0.92 &    0.97 &  0.98 \\
 &  \sysname-M &     0.99 &  0.98 &  1.00 &  1.00 &    0.98 &  0.98 \\
 \hline
\multirow{4}{*}{Llama-70B} &     Self Reminder &     0.51 &  0.85 &  0.84 &  0.89 &    0.93 &  0.92 \\
 &       Safe Prompt &     0.87 &  0.70 &  0.89 &  0.91 &    0.93 &  0.96 \\
 &  GPT Paraphrasing &     0.91 &  0.95 &  0.94 &  0.93 &    0.97 &  0.97 \\
 &         \sysname &     0.96 &  0.98 &  0.98 &  0.98 &    0.98 &  0.99 \\
 &  \sysname-M &     1.00 &  1.00 &  0.99 &  1.00 &    0.99 &  0.99 \\
\hline\hline
\end{tabular}
    \caption{The detailed accuracy of the evaluation}
    \label{tab:acc_details}
\end{table}

\begin{figure}[htbp]
  \centering
    \subfloat[\scriptsize{Vicuna-1.5}]{\includegraphics[width=0.5\textwidth]{figures/adaptive-Vicuna-1.5.pdf}}
    \subfloat[\scriptsize{Llama-2}]{\includegraphics[width=0.5\textwidth]{figures/adaptive-Llama-2.pdf}}
    \\
  \caption{
  We consider different schemes' defense effectiveness against adaptive attacks. The results indicate that our proposed \sysname (with randomization) can drop the ASR of adaptive attacks within 10\%.
  }
  \label{fig:adaptive}
  \vspace{0.2in}
\end{figure}
